Tailoring Stakeholder Interests to Task-Oriented Functional Requirements

Without a specific functional context, non-functional requirements can only be approached as cross-cutting concerns and treated uniformly across all features of an application. This neglects, however, the heterogeneity of non-functional requirements that arises from stakeholder interests and the distinct functional scopes of software systems, which mutually influence how these non-functional requirements have to be satisfied. Earlier studies showed that the different types and objectives of non-functional requirements result in either vague or unbalanced specification of non-functional requirements. We propose a task analytic approach for eliciting and modeling user tasks to approach the stakeholders' pursued interests towards the software product. Stakeholder interests are structurally related to user tasks and each interest can be specified individually as a constraint of a specific user task. These constraints support DevOps teams with important guidance on how the interest of the stakeholder can be satisfied in the software lifecycle sufficiently. We propose a structured approach, intertwining task-oriented functional requirements with non-functional stakeholder interests to specify constraints on the level of user tasks. We also present results of a case study with domain experts, which reveals that our task modeling and interest-tailoring method increases the comprehensibility of non-functional requirements as well as their impact on the functional requirements, i.e., the users' tasks.

==> task_details_table.tex <==
\begin{table*} \scriptsize 
\centering
\caption{User and System Task Details.}\label{tab:user_system_task_details}
\bgroup
\def\arraystretch{1.5}% 
\begin{tabular}{|p{1.7cm}|p{4.05cm}|p{6cm}|}
\hline
\cellcolor{lightgray}\textbf{Subtask ID} & \cellcolor{lightgray}\textbf{User Intention} & \cellcolor{lightgray}\textbf{System Responsibility}\\
\hline
1 & Entering title of book & Providing suggestions for book titles \\
\hline
2 & & Searching for book 
\begin{itemize}[nosep]
	\item Search by title and for similar books \vspace*{-\baselineskip}
\end{itemize} \\
\hline
3 & & Displaying results
\begin{itemize}[nosep]
\item Format the list of matches
\item Display exact matching and similar books \vspace*{-\baselineskip}
\end{itemize} \\
\hline
4 & Selecting a book from a list of \newline matches & \\
\hline
5 & & Displaying details of selected book \\
\hline
\end{tabular}
\egroup
\end{table*}
\begin{table*} \scriptsize 
\centering
\caption{Pre-/Post-Conditions and Information Objects of the Subtasks.}\label{tab:pre_post_conditions}
\bgroup
\def\arraystretch{1.5}% 
\begin{tabular}{|p{1.7cm}|p{3cm}|p{4.15cm}|p{2.8cm}|}
\hline
\cellcolor{lightgray}\textbf{Subtask ID} & \cellcolor{lightgray}\textbf{Pre-Condition} & \cellcolor{lightgray}\textbf{Information Object} & \cellcolor{lightgray}\textbf{Post-Condition}\\
\hline
1 & Customer logged in & \vspace{-6pt} \begin{itemize}
\item Search term \textit{(in)}
\item List of book titles for \newline auto-completion \textit{(out)} \vspace*{-\baselineskip}
\end{itemize} & \\
\hline
2 & & List of matches with title, \newline author, cover, and year \textit{(out)} & \\
\hline
3 & & List of matches with title, \newline author, cover, and year \textit{(in)} & \\
\hline
4 & & Selected book \textit{(out)} & \\
\hline
5 & & Selected book \textit{(in)} & Search terms saved \newline in profile \\
\hline
\end{tabular}
\egroup
\end{table*}

==> terminology.tex <==
\label{terminology}
\ploe{This}{Vielleicht keine eigene section dafür, sondern in II einarbeiten} section clarifies the terms and theoretical background of this paper. \resolved{\ploe{and theoretical background of}{Ist das wirklich ein theoretischer Hintergrund? Sollten wir nicht besser schreiben: 'used in'}this paper. }
\begin{itemize}
\iffalse\item	\textit{Satisfice:} is a portmanteau of \textit{satisfy} and \textit{suffice}. It expresses the intention to satisfy a requirement in a complex system in a sufficient but not optimal way - so that a multitude of goals can be satisfied concurrently. \fi
\item	\textit{Task:} is a sequence of actions that people perform to attain a goal. Tasks differ in associated goals, input modalities (e.g., software-based, in-person), and the actions they require for their attainment \cite{annett_hierarchical_2003}. A task can also be seen as the execution sequence of different software features, i.e., the interpretation of results of a feature and the decision which feature to use next.
\iffalse
\item	\textit{Task Analysis:} elicits the actions, sequences, decision points, knowledge, and sensory information required to attain a goal. Task analysis methods provide structured techniques for information gathering and differ in the granularity and type of information they elicit. While hierarchical task analysis methods focus on repetitive decomposition of human tasks, cognitive analysis methods support knowledge elicitation and exploration. \fi
\item	\textit{Hierarchical Task Analysis:} breaks down a task into goals, subgoals, plans, and operations, focusing on the structure and decomposition of the task into a hierarchy of subtasks in sequential order of tasks so that the goal can be attained.
\item	\textit{Feature:} is a specific functionality or capability that a software system provides \cite{bourque_guide_2014} to attain a goal with it. In this work we refer to features as concrete software implementations which realize the actions that are required to implement a task.
\item\textit{Constraint:} is a refinement and operationalization of a non-functional requirement that can be validated for fulfillment. Constraints can be further classified as performance, maintainability, safety, reliability, security, or interoperability constraints \cite{bourque_guide_2014}. Tasks and their constraints cannot be seen in isolation as constraints influence software design and architectural decisions \cite{broy_rethinking_2015}.
\item \textit{Stakeholder Interests:} extend the primarily technical notion of non-functional requirements to also capture relevant non-engineering interests of stakeholders. These interests are still unsatisfactorily covered by existing, solely technically oriented standards such as ISO/IEC 29148:2011 \cite{noauthor_iso/iec/ieee_2011-1} or ISO/IEC 25030:2007 \cite{noauthor_iso/iec/ieee_2018}, which often results in non-functional requirements being only vaguely elicited. A classification scheme of possible interests is given in section \ref{interests_classification_schema}.
\end{itemize}
